PCGRL+: Scaling, Control and Generalization in Reinforcement Learning Level Generators

Procedural Content Generation via Reinforcement Learning (PCGRL) has been introduced as a means by which controllable designer agents can be trained based only on a set of computable metrics acting as a proxy for the level's quality and key characteristics. While PCGRL offers a unique set of affordances for game designers, it is constrained by the compute-intensive process of training RL agents, and has so far been limited to generating relatively small levels. To address this issue of scale, we implement several PCGRL environments in Jax so that all aspects of learning and simulation happen in parallel on the GPU, resulting in faster environment simulation; removing the CPU-GPU transfer of information bottleneck during RL training; and ultimately resulting in significantly improved training speed. We replicate several key results from prior works in this new framework, letting models train for much longer than previously studied, and evaluating their behavior after 1 billion timesteps. Aiming for greater control for human designers, we introduce randomized level sizes and frozen "pinpoints" of pivotal game tiles as further ways of countering overfitting. To test the generalization ability of learned generators, we evaluate models on large, out-of-distribution map sizes, and find that partial observation sizes learn more robust design strategies.

==> figs_OLD/bs_binary_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & \multicolumn{3}{c}{mean ep reward} \\
eval map width & 16 & 24 & 32 \\
max. board scans &  &  &  \\
\midrule
1 & 89.66 ± 8.17 & \textbf{119.07} ± \textbf{8.54} & \textbf{156.69} ± \textbf{2.37} \\
5 & \textbf{118.31} ± \textbf{12.17} & 105.32 ± 4.11 & 135.91 ± 6.30 \\
10 & 116.69 ± 11.66 & 105.94 ± 29.37 & 138.18 ± 26.48 \\
\bottomrule
\end{tabular}


==> tables/act_shape_conv2_dungeon_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
act shape &  &  &  &  \\
\midrule
(1, 1) & \textbf{7.51} ± \textbf{1.10} & 30.35 ± 3.35 & \textbf{91.37} ± \textbf{2.29} & \textbf{132.96} ± \textbf{5.16} \\
(2, 2) & 1.14 ± 2.28 & 29.80 ± 3.77 & 44.13 ± 55.46 & 63.73 ± 80.85 \\
(3, 3) & 5.38 ± 0.41 & 30.65 ± 0.74 & 85.41 ± 3.51 & 125.03 ± 5.30 \\
(4, 4) & 4.54 ± 0.80 & 30.96 ± 3.51 & 88.07 ± 4.06 & 127.64 ± 4.11 \\
(5, 5) & -2.21 ± 2.61 & \textbf{31.49} ± \textbf{3.58} & 85.49 ± 1.63 & 127.62 ± 1.45 \\
(6, 6) & 4.53 ± 2.69 & 31.39 ± 3.29 & 88.46 ± 4.01 & 122.13 ± 4.71 \\
\bottomrule
\end{tabular}

\label{tab:act_shape_conv2_dungeon_eval_map_width}

==> tables/act_shape_conv2_dungeon_eval_randomize_map_shap_map_width.tex <==
\centering
\adjustbox{max width=\textwidth}{%
\begin{tabular}{lllll|llll}
\toprule
 & \multicolumn{8}{c}{mean ep reward} \\
rand. map shape & \multicolumn{4}{c}{False} & \multicolumn{4}{c}{True} \\
eval map width & 8 & 16 & 24 & 32 & 8 & 16 & 24 & 32 \\
\toprule
act shape &  &  &  &  &  &  &  &  \\
\midrule
(1, 1) & 18.04 ± 0.66 & \textbf{269.86} ± \textbf{29.98} & 273.20 ± 4.02 & 492.98 ± 6.93 & \textbf{7.51} ± \textbf{1.08} & 30.35 ± 3.28 & \textbf{91.37} ± \textbf{2.24} & \textbf{132.96} ± \textbf{5.04} \\
(2, 2) & 12.76 ± 2.84 & 240.45 ± 83.15 & 104.32 ± 195.66 & 213.21 ± 359.19 & 1.14 ± 2.23 & 29.80 ± 3.68 & 44.13 ± 54.24 & 63.73 ± 79.07 \\
(3, 3) & 18.09 ± 1.52 & 227.02 ± 78.03 & \textbf{274.81} ± \textbf{6.22} & 490.98 ± 6.73 & 5.38 ± 0.40 & 30.65 ± 0.72 & 85.41 ± 3.43 & 125.03 ± 5.18 \\
(4, 4) & \textbf{20.39} ± \textbf{1.84} & 206.56 ± 1.27 & 267.85 ± 16.15 & 486.52 ± 19.52 & 4.54 ± 0.78 & 30.96 ± 3.43 & 88.07 ± 3.97 & 127.64 ± 4.02 \\
(5, 5) & 5.34 ± 3.88 & 216.11 ± 32.57 & 274.29 ± 7.58 & \textbf{506.88} ± \textbf{10.30} & -2.21 ± 2.55 & \textbf{31.49} ± \textbf{3.50} & 85.49 ± 1.60 & 127.62 ± 1.42 \\
(6, 6) & 16.62 ± 1.24 & 146.69 ± 43.82 & 268.74 ± 13.81 & 470.19 ± 15.92 & 4.53 ± 2.63 & 31.39 ± 3.21 & 88.46 ± 3.92 & 122.13 ± 4.60 \\
\bottomrule
\end{tabular}

\label{tab:act_shape_conv2_dungeon_eval_randomize_map_shap_map_width}
}

==> tables/arf_conv_binary_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
arf size &  &  &  &  \\
\midrule
3 & 10.67 ± 0.83 & 27.10 ± 1.37 & 42.72 ± 2.27 & 65.83 ± 4.08 \\
5 & 9.77 ± 0.38 & 27.52 ± 2.16 & 42.17 ± 3.90 & 62.77 ± 3.83 \\
8 & \textbf{11.19} ± \textbf{0.50} & \textbf{33.38} ± \textbf{2.44} & \textbf{52.05} ± \textbf{4.61} & \textbf{77.83} ± \textbf{6.44} \\
16 & 10.92 ± 0.58 & 30.41 ± 2.71 & 46.51 ± 4.58 & 66.45 ± 10.05 \\
31 & 8.85 ± 2.00 & 25.69 ± 2.45 & 42.06 ± 4.42 & 63.57 ± 4.70 \\
\bottomrule
\end{tabular}

\label{tab:arf_conv_binary_eval_map_width}

==> tables/arf_seqnca_dungeon_eval_map_width.tex <==
\centering
\begin{tabular}{llll}
\toprule
 & \multicolumn{3}{c}{mean ep reward} \\
eval map width & 16 & 24 & 32 \\
\toprule
arf size &  &  &  \\
\midrule
3 & 36.53 ± 1.32 & 97.95 ± 3.09 & 137.21 ± 2.83 \\
5 & 37.87 ± 3.87 & 102.92 ± 6.10 & \textbf{139.91} ± \textbf{5.59} \\
8 & \textbf{40.76} ± \textbf{1.95} & \textbf{104.14} ± \textbf{9.08} & 139.80 ± 6.37 \\
16 & 36.08 ± 2.91 & 95.29 ± 2.81 & 135.89 ± 2.29 \\
31 & 32.77 ± 2.15 & 92.07 ± 2.34 & 132.09 ± 3.37 \\
\bottomrule
\end{tabular}


\label{tab:arf_seqnca_dungeon_eval_map_width}

==> tables/bs_binary_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
max. board scans &  &  &  &  \\
\midrule
1 & 18.43 ± 1.62 & 89.66 ± 8.05 & \textbf{119.07} ± \textbf{8.41} & \textbf{156.69} ± \textbf{2.33} \\
5 & 20.17 ± 1.42 & \textbf{118.31} ± \textbf{11.98} & 105.32 ± 4.05 & 135.91 ± 6.20 \\
10 & \textbf{26.36} ± \textbf{4.33} & 116.69 ± 11.48 & 105.94 ± 28.92 & 138.18 ± 26.07 \\
\bottomrule
\end{tabular}


==> tables/diffshape_pinpoint_maze_emptystart_eval_map_width.tex <==
\centering
\begin{tabular}{llllll}
\toprule
 &  & \multicolumn{4}{c}{mean ep reward} \\
 & eval map width & 8 & 16 & 24 & 32 \\
\toprule
randomize map shape & obs size &  &  &  &  \\
\midrule
\multirow[t]{4}{*}{False} & 8 & 1.23 ± 0.61 & 4.82 ± 1.62 & 9.57 ± 4.50 & 6.10 ± 7.60 \\
 & 16 & 0.27 ± 0.49 & -1.28 ± 4.60 & -3.15 ± 2.94 & -8.14 ± 3.16 \\
 & 24 & 0.87 ± 0.65 & 1.07 ± 1.10 & 1.11 ± 0.94 & 0.79 ± 0.47 \\
 & 31 & 0.93 ± 0.03 & -2.33 ± 3.96 & -5.97 ± 5.34 & -6.71 ± 7.07 \\
\cline{1-6}
\multirow[t]{4}{*}{True} & 8 & \textbf{6.61} ± \textbf{0.17} & 20.09 ± 2.76 & \textbf{26.11} ± \textbf{4.17} & \textbf{25.12} ± \textbf{1.90} \\
 & 16 & 5.93 ± 0.40 & \textbf{21.75} ± \textbf{1.80} & 16.57 ± 2.85 & 16.87 ± 5.08 \\
 & 24 & 5.08 ± 0.77 & 18.31 ± 1.97 & 5.67 ± 3.79 & -0.84 ± 3.73 \\
 & 31 & 3.76 ± 0.21 & 18.69 ± 0.56 & 3.82 ± 1.77 & -0.68 ± 2.24 \\
\cline{1-6}
\bottomrule
\end{tabular}

\label{tab:diffshape_pinpoint_maze_emptystart_eval_map_width}

==> tables/n_envs_to_fps_jax_train.tex <==
\centering
\begin{tabular}{lrrrrrrr}
    n. envs & 1 & 10 & 50 & 100 & 200 & 400 & 600 \\ 
    \hline
    binary & 256 & 1,256 & 1,098 & 3,993 & 6,076 & 7,814 & 8,943 \\ 
    maze & 471 & 2,099 & 6,159 & 8,039 & 9,319 & 9,456 & 10,961  \\ 
    dungeon & 292 & 1,463 & 4,042 & 5,375 & 6,851 & 7,502 & 8,798 \\ 
\end{tabular}

==> tables/n_envs_to_fps_old_codebase.tex <==
\centering
\begin{tabular}{lrrrrrrr}
    n. envs & 1 & 10 & 50 & 100 & 200 & 400 & 600 \\ 
    \hline
    binary & 188.681 & 420.136 & 519.905 & 524.195 & 525.244 & 528.972 & 521.994 \\ 
    zelda & 206.452 & 416.429 & 504.844 & 510.768 & 509.398 & 511.37 & 496.257 \\ 
\end{tabular}

==> tables/obss_conv2_dungeon_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
obs size &  &  &  &  \\
\midrule
15 & 6.19 ± 0.34 & 38.48 ± 0.39 & 96.22 ± 2.07 & \textbf{140.16} ± \textbf{4.93} \\
20 & 7.06 ± 0.63 & 37.56 ± 1.93 & \textbf{97.18} ± \textbf{1.53} & 135.03 ± 2.04 \\
25 & \textbf{8.64} ± \textbf{1.74} & \textbf{39.44} ± \textbf{3.25} & 96.55 ± 0.78 & 136.51 ± 1.15 \\
31 & 7.51 ± 1.10 & 30.35 ± 3.35 & 91.37 ± 2.29 & 132.96 ± 5.16 \\
\bottomrule
\end{tabular}

\label{tab:obss_conv2_dungeon_eval_map_width}

==> tables/obss_dungeon_conv2_ctrl_path_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
obs size &  &  &  &  \\
\midrule
3 & 7.70 ± 1.60 & 35.65 ± 2.77 & 99.90 ± 4.20 & 138.22 ± 3.78 \\
5 & 8.40 ± 1.50 & \textbf{37.56} ± \textbf{1.78} & \textbf{100.57} ± \textbf{5.61} & 139.29 ± 3.54 \\
8 & 7.23 ± 0.90 & 36.82 ± 1.18 & 99.73 ± 1.76 & \textbf{145.10} ± \textbf{4.18} \\
16 & 5.34 ± 0.90 & 36.46 ± 1.62 & 98.90 ± 3.18 & 136.70 ± 1.56 \\
31 & \textbf{8.60} ± \textbf{0.87} & 35.48 ± 0.39 & 93.54 ± 2.67 & 136.60 ± 3.13 \\
\bottomrule
\end{tabular}

\label{tab:obss_dungeon_conv2_ctrl_path_eval_map_width}

==> tables/obss_hiddims_dungeon_conv2_ctrl_path_eval_map_width.tex <==
\centering
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{c}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
\toprule
obs size hid dims &  &  &  &  \\
\midrule
3 & \textbf{10.89} ± \textbf{2.25} & 39.89 ± 1.96 & \textbf{103.75} ± \textbf{0.97} & 141.59 ± 2.15 \\
5 & 9.87 ± 0.62 & 41.39 ± 3.78 & 103.48 ± 5.53 & \textbf{145.19} ± \textbf{5.62} \\
8 & 8.53 ± 0.17 & 38.99 ± 2.94 & 103.19 ± 2.03 & 139.42 ± 0.83 \\
16 & 5.80 ± 0.15 & \textbf{44.19} ± \textbf{3.53} & 100.01 ± 6.68 & 135.75 ± 6.38 \\
31 & 5.03 ± 0.83 & 31.03 ± 1.33 & 92.21 ± 3.58 & 133.53 ± 1.98 \\
\bottomrule
\end{tabular}

\label{tab:obss_hiddims_dungeon_conv2_ctrl_path_eval_map_width}

==> tables_OLD/act_shape_conv2_dungeon_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & mean ep reward & mean min ep loss & min min ep loss \\
act shape &  &  &  \\
\midrule
(1, 1) & \textbf{250.07} & \textbf{0.03} & \textbf{0.00} \\
(2, 2) & 187.01 & 0.04 & \textbf{0.00} \\
(3, 3) & 162.68 & 0.04 & \textbf{0.00} \\
(4, 4) & 176.38 & 0.04 & \textbf{0.00} \\
(5, 5) & 138.07 & 0.05 & \textbf{0.00} \\
(6, 6) & 96.79 & 0.05 & \textbf{0.00} \\
\bottomrule
\end{tabular}


==> tables_OLD/act_shape_conv2_dungeon_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{r}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
act shape &  &  &  &  \\
\midrule
(1, 1) & \textbf{7.51} ± \textbf{1.10} & 30.35 ± 3.35 & \textbf{91.37} ± \textbf{2.29} & \textbf{132.96} ± \textbf{5.16} \\
(2, 2) & 1.14 ± 2.28 & 29.80 ± 3.77 & 44.13 ± 55.46 & 63.73 ± 80.85 \\
(3, 3) & 5.38 ± 0.41 & 30.65 ± 0.74 & 85.41 ± 3.51 & 125.03 ± 5.30 \\
(4, 4) & 4.54 ± 0.80 & 30.96 ± 3.51 & 88.07 ± 4.06 & 127.64 ± 4.11 \\
(5, 5) & -2.21 ± 2.61 & \textbf{31.49} ± \textbf{3.58} & 85.49 ± 1.63 & 127.62 ± 1.45 \\
(6, 6) & 4.53 ± 2.69 & 31.39 ± 3.29 & 88.46 ± 4.01 & 122.13 ± 4.71 \\
\bottomrule
\end{tabular}


==> tables_OLD/act_shape_seqnca_dungeon_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & mean ep reward & mean min ep loss & min min ep loss \\
act shape &  &  &  \\
\midrule
(1, 1) & \textbf{294.90} & \textbf{0.02} & \textbf{0.00} \\
(2, 2) & 206.17 & 0.04 & \textbf{0.00} \\
(3, 3) & 228.76 & 0.04 & \textbf{0.00} \\
(4, 4) & 167.20 & 0.05 & \textbf{0.00} \\
(5, 5) & 99.68 & 0.06 & \textbf{0.00} \\
(6, 6) & 73.89 & 0.06 & \textbf{0.00} \\
\bottomrule
\end{tabular}


==> tables_OLD/act_shape_seqnca_dungeon_diff_size_stats_size_16_concise.tex <==
\begin{tabular}{lllll}
\toprule
 &  & mean ep reward & mean min ep loss & min min ep loss \\
act shape & eval map width &  &  &  \\
\midrule
\multirow[t]{3}{*}{(1, 1)} & 16 & \textbf{313.26} & 0.02 & \textbf{0.00} \\
 & 18 & 179.91 & 0.05 & \textbf{0.00} \\
 & 20 & 205.08 & 0.05 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{(2, 2)} & 16 & 191.20 & 0.05 & \textbf{0.00} \\
 & 18 & 178.37 & 0.06 & \textbf{0.00} \\
 & 20 & 217.64 & 0.06 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{(3, 3)} & 16 & 136.07 & 0.05 & \textbf{0.00} \\
 & 18 & 134.15 & 0.06 & \textbf{0.00} \\
 & 20 & 180.19 & 0.06 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{(4, 4)} & 16 & 159.77 & 0.05 & \textbf{0.00} \\
 & 18 & 147.55 & 0.06 & \textbf{0.00} \\
 & 20 & 195.55 & 0.06 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{(5, 5)} & 16 & 103.43 & 0.06 & \textbf{0.00} \\
 & 18 & 104.84 & 0.07 & \textbf{0.00} \\
 & 20 & 140.35 & 0.06 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{(6, 6)} & 16 & 67.48 & 0.06 & \textbf{0.00} \\
 & 18 & 55.36 & \textbf{0.07} & \textbf{0.00} \\
 & 20 & 89.65 & 0.07 & \textbf{0.00} \\
\cline{1-5}
\bottomrule
\end{tabular}


==> tables_OLD/action_patch.tex <==
\begin{tabular}{|c|c|c|c|}
\toprule
 &  & episode reward max & episode reward mean \\
model & act window &  &  \\
\midrule
\multirow[c]{6}{*}{Default} & (16, 16) & 65.67 ± 3.79 & 8.22 ± 1.62 \\
 & (8, 8) & 90.67 ± 4.04 & 40.40 ± 1.77 \\
 & (6, 6) & 100.00 ± 13.08 & 58.49 ± 15.06 \\
 & (4, 4) & 122.00 ± 6.56 & 82.96 ± 11.66 \\
 & (2, 2) & 116.67 ± 6.81 & 71.55 ± 3.68 \\
 & (1, 1) & 98.33 ± 2.52 & 58.08 ± 1.49 \\
\cline{1-4}
\multirow[c]{6}{*}{SeqNCA} & (16, 16) & 76.00 ± 5.57 & 27.12 ± 1.27 \\
 & (8, 8) & 90.33 ± 7.77 & 51.47 ± 6.84 \\
 & (6, 6) & 92.67 ± 4.16 & 49.59 ± 6.69 \\
 & (4, 4) & 96.33 ± 10.02 & 56.01 ± 6.80 \\
 & (2, 2) & \bfseries 149.00 ± 26.87 & \bfseries 108.92 ± 15.03 \\
 & (1, 1) & 137.00 ± 30.81 & 97.70 ± 31.41 \\
\cline{1-4}
\bottomrule
\end{tabular}

% 100 eps

==> tables_OLD/arf_conv_binary_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{r}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
arf size &  &  &  &  \\
\midrule
3 & 10.67 ± 0.83 & 27.10 ± 1.37 & 42.72 ± 2.27 & 65.83 ± 4.08 \\
5 & 9.77 ± 0.38 & 27.52 ± 2.16 & 42.17 ± 3.90 & 62.77 ± 3.83 \\
8 & \textbf{11.19} ± \textbf{0.50} & \textbf{33.38} ± \textbf{2.44} & \textbf{52.05} ± \textbf{4.61} & \textbf{77.83} ± \textbf{6.44} \\
16 & 10.92 ± 0.58 & 30.41 ± 2.71 & 46.51 ± 4.58 & 66.45 ± 10.05 \\
31 & 8.85 ± 2.00 & 25.69 ± 2.45 & 42.06 ± 4.42 & 63.57 ± 4.70 \\
\bottomrule
\end{tabular}


==> tables_OLD/arf_seqnca_binary_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & mean ep reward & mean min ep loss & min min ep loss \\
arf size &  &  &  \\
\midrule
3 & 91.62 & 0.15 & \textbf{0.00} \\
5 & 102.25 & 0.14 & \textbf{0.00} \\
8 & 110.98 & 0.12 & \textbf{0.00} \\
16 & \textbf{131.39} & \textbf{0.03} & \textbf{0.00} \\
31 & 128.54 & 0.05 & \textbf{0.00} \\
\bottomrule
\end{tabular}


==> tables_OLD/arf_seqnca_dungeon_diff_size_stats_size_16_concise.tex <==
\begin{tabular}{lllll}
\toprule
 &  & mean ep reward & mean min ep loss & min min ep loss \\
arf size & eval map width &  &  &  \\
\midrule
\multirow[t]{3}{*}{3} & 16 & 194.12 & 0.04 & \textbf{0.00} \\
 & 18 & 192.71 & 0.04 & \textbf{0.00} \\
 & 20 & 204.36 & 0.05 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{5} & 16 & 201.90 & 0.04 & \textbf{0.00} \\
 & 18 & 207.01 & 0.04 & \textbf{0.00} \\
 & 20 & 213.17 & 0.05 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{8} & 16 & 257.14 & 0.03 & \textbf{0.00} \\
 & 18 & 299.51 & 0.03 & \textbf{0.00} \\
 & 20 & 307.94 & 0.04 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{16} & 16 & 288.30 & 0.02 & \textbf{0.00} \\
 & 18 & 281.52 & 0.03 & \textbf{0.00} \\
 & 20 & 217.10 & 0.05 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{31} & 16 & \textbf{313.26} & 0.02 & \textbf{0.00} \\
 & 18 & 179.91 & 0.05 & \textbf{0.00} \\
 & 20 & 205.08 & \textbf{0.05} & \textbf{0.00} \\
\cline{1-5}
\bottomrule
\end{tabular}


==> tables_OLD/bs_binary_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & mean ep reward & mean loss & min. loss \\
max. board scans &  &  &  \\
\midrule
1 & 89.66 & 15.80\% & 12.05\% \\
5 & \textbf{118.31} & \textbf{9.69\%} & 5.78\% \\
10 & 116.69 & 9.84\% & \textbf{4.06\%} \\
\bottomrule
\end{tabular}


==> tables_OLD/bs_binary_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{llll}
\toprule
 & \multicolumn{3}{r}{mean ep reward} \\
eval map width & 16 & 24 & 32 \\
max. board scans &  &  &  \\
\midrule
1 & 89.66 ± 8.17 & \textbf{119.07} ± \textbf{8.54} & \textbf{156.69} ± \textbf{2.37} \\
5 & \textbf{118.31} ± \textbf{12.17} & 105.32 ± 4.11 & 135.91 ± 6.30 \\
10 & 116.69 ± 11.66 & 105.94 ± 29.37 & 138.18 ± 26.48 \\
\bottomrule
\end{tabular}


==> tables_OLD/combine_action_patch_seqnca.tex <==
\begin{tabular}{|c|c|c|c|c|}
\toprule
 &  &  & episode reward max & episode reward mean \\
model & act window & model patch width &  &  \\
\midrule
\multirow[c]{10}{*}{SeqNCA} & (1, 1) & 3 & 137.00 ± 30.81 & 97.70 ± 31.41 \\
\cline{2-5}
 & \multirow[c]{3}{*}{(2, 2)} & 3 & 149.00 ± 26.87 & 108.92 ± 15.03 \\
 &  & 5 & 148.67 ± 10.69 & 106.93 ± 16.48 \\
 &  & 7 & 132.00 ± 25.24 & 98.00 ± 26.15 \\
\cline{2-5}
 & \multirow[c]{3}{*}{(4, 4)} & 3 & 96.33 ± 10.02 & 56.01 ± 6.80 \\
 &  & 5 & 93.33 ± 9.29 & 57.93 ± 8.57 \\
 &  & 7 & 90.33 ± 2.52 & 51.50 ± 2.70 \\
\cline{2-5}
 & \multirow[c]{3}{*}{(6, 6)} & 3 & 92.67 ± 4.16 & 49.59 ± 6.69 \\
 &  & 5 & 62.00 ± 4.58 & 31.30 ± 7.14 \\
 &  & 7 & 79.67 ± 7.77 & 30.83 ± 6.44 \\
\cline{1-5} \cline{2-5}
\bottomrule
\end{tabular}


==> tables_OLD/combine_action_patch_static_walls_default.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\toprule
 &  &  &  & episode reward max & episode reward mean & episode reward min & path-length max & path-length mean & path-length min \\
model & act window & n static walls & static prob &  &  &  &  &  &  \\
\midrule
\multirow[c]{11}{*}{Default} & \multirow[c]{6}{*}{(4, 4)} & \multirow[c]{2}{*}{3} & 0.0 & 85.00 ± 13.45 & 46.90 ± 2.78 & 10.00 ± 11.14 & 65.33 ± 2.89 & 51.93 ± 1.07 & 36.67 ± 5.51 \\
 &  &  & 0.1 & 76.67 ± 7.77 & 39.27 ± 8.05 & 5.67 ± 3.21 & 66.00 ± 1.73 & 46.60 ± 3.72 & 32.33 ± 2.08 \\
\cline{3-10}
 &  & \multirow[c]{2}{*}{5} & 0.0 & 89.33 ± 8.62 & 50.80 ± 1.21 & 9.00 ± 6.08 & 64.00 ± 6.08 & 46.00 ± 0.36 & 26.33 ± 2.31 \\
 &  &  & 0.1 & 62.00 ± 17.52 & 35.97 ± 4.99 & 2.67 ± 12.01 & 55.00 ± 13.89 & 40.03 ± 8.21 & 22.67 ± 7.02 \\
\cline{3-10}
 &  & \multirow[c]{2}{*}{7} & 0.0 & 72.33 ± 11.15 & 45.30 ± 7.71 & 11.67 ± 15.95 & 59.33 ± 4.62 & 43.17 ± 4.24 & 29.00 ± 1.73 \\
 &  &  & 0.1 & 70.00 ± 3.46 & 35.77 ± 7.76 & -12.33 ± 16.04 & 54.33 ± 6.35 & 41.97 ± 2.47 & 31.67 ± 2.89 \\
\cline{2-10} \cline{3-10}
 & \multirow[c]{5}{*}{(2, 2)} & \multirow[c]{2}{*}{3} & 0.0 & 77.33 ± 10.50 & 46.17 ± 7.00 & 2.33 ± 7.64 & 58.67 ± 5.69 & 44.33 ± 3.33 & 29.67 ± 3.21 \\
 &  &  & 0.1 & 83.67 ± 6.35 & 50.13 ± 1.26 & 17.33 ± 8.14 & 57.00 ± 3.00 & 48.43 ± 2.90 & 32.33 ± 0.58 \\
\cline{3-10}
 &  & \multirow[c]{2}{*}{5} & 0.0 & 81.00 ± 11.14 & 52.40 ± 2.13 & 7.00 ± 5.29 & 60.67 ± 6.43 & 49.67 ± 3.70 & 32.33 ± 8.02 \\
 &  &  & 0.1 & 75.67 ± 4.73 & 39.50 ± 6.75 & -0.67 ± 16.44 & 57.67 ± 4.04 & 44.70 ± 3.05 & 29.67 ± 7.64 \\
\cline{3-10}
 &  & 7 & 0.0 & 76.00 ± 9.90 & 54.75 ± 0.78 & -6.50 ± 28.99 & 61.50 ± 3.54 & 49.45 ± 2.19 & 36.00 ± 7.07 \\
\cline{1-10} \cline{2-10} \cline{3-10}
\bottomrule
\end{tabular}


==> tables_OLD/different_size_eval_binary_conv_bs4_vrf31_arfsweep.tex <==
\begin{tabular}{lll}
\toprule
 &  & mean ep reward \\
arf size & eval map width &  \\
\midrule
\multirow[t]{3}{*}{3} & 16 & 68.45 \\
 & 18 & 80.54 \\
 & 20 & 98.81 \\
\cline{1-3}
\multirow[t]{3}{*}{5} & 16 & 75.45 \\
 & 18 & 89.52 \\
 & 20 & 106.97 \\
\cline{1-3}
\multirow[t]{3}{*}{8} & 16 & 94.93 \\
 & 18 & 107.62 \\
 & 20 & 130.26 \\
\cline{1-3}
\multirow[t]{3}{*}{16} & 16 & 99.92 \\
 & 18 & 110.76 \\
 & 20 & \textbf{132.23} \\
\cline{1-3}
\multirow[t]{3}{*}{31} & 16 & 114.11 \\
 & 18 & 106.11 \\
 & 20 & 131.18 \\
\cline{1-3}
\bottomrule
\end{tabular}

==> tables_OLD/different_size_seqnca_eval_binary_conv_bs4_vrf31_arfsweep.tex <==
\begin{tabular}{lllll}
\toprule
 &  & mean ep reward & mean min ep loss & min min ep loss \\
arf size & eval map width &  &  &  \\
\midrule
\multirow[t]{3}{*}{3} & 16 & 87.94 & 0.18 & \textbf{0.00} \\
 & 18 & 103.77 & 0.20 & \textbf{0.00} \\
 & 20 & 123.16 & 0.21 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{5} & 16 & 102.51 & 0.13 & \textbf{0.00} \\
 & 18 & 126.75 & 0.15 & \textbf{0.00} \\
 & 20 & \textbf{152.15} & 0.15 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{8} & 16 & 107.80 & 0.12 & \textbf{0.00} \\
 & 18 & 124.39 & 0.16 & \textbf{0.00} \\
 & 20 & 133.99 & 0.19 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{16} & 16 & 114.04 & 0.10 & \textbf{0.00} \\
 & 18 & 127.11 & 0.15 & \textbf{0.00} \\
 & 20 & 144.89 & 0.18 & \textbf{0.00} \\
\cline{1-5}
\multirow[t]{3}{*}{31} & 16 & 134.22 & 0.03 & \textbf{0.00} \\
 & 18 & 84.93 & 0.22 & \textbf{0.00} \\
 & 20 & 90.05 & \textbf{0.28} & \textbf{0.00} \\
\cline{1-5}
\bottomrule
\end{tabular}


==> tables_OLD/diffshape_pinpoint_maze_emptystart_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{llllll}
\toprule
 &  & \multicolumn{4}{r}{mean ep reward} \\
 & eval map width & 8 & 16 & 24 & 32 \\
 \midrule
randomize map shape & obs size &  &  &  &  \\
\midrule
\multirow[t]{4}{*}{False} & 8 & 1.23 ± 0.61 & 4.82 ± 1.62 & 9.57 ± 4.50 & 6.10 ± 7.60 \\
 & 16 & 0.27 ± 0.49 & -1.28 ± 4.60 & -3.15 ± 2.94 & -8.14 ± 3.16 \\
 & 24 & 0.87 ± 0.65 & 1.07 ± 1.10 & 1.11 ± 0.94 & 0.79 ± 0.47 \\
 & 31 & 0.93 ± 0.03 & -2.33 ± 3.96 & -5.97 ± 5.34 & -6.71 ± 7.07 \\
\cline{1-6}
\multirow[t]{4}{*}{True} & 8 & \textbf{6.61} ± \textbf{0.17} & 20.09 ± 2.76 & \textbf{26.11} ± \textbf{4.17} & \textbf{25.12} ± \textbf{1.90} \\
 & 16 & 5.93 ± 0.40 & \textbf{21.75} ± \textbf{1.80} & 16.57 ± 2.85 & 16.87 ± 5.08 \\
 & 24 & 5.08 ± 0.77 & 18.31 ± 1.97 & 5.67 ± 3.79 & -0.84 ± 3.73 \\
 & 31 & 3.76 ± 0.21 & 18.69 ± 0.56 & 3.82 ± 1.77 & -0.68 ± 2.24 \\
\cline{1-6}
\bottomrule
\end{tabular}


==> tables_OLD/n_agents.tex <==
\begin{tabular}{|c|c|c|c|c|}
\toprule
 &  &  & episode reward max & episode reward mean \\
multiagent & show agents & n  agents &  &  \\
\midrule
\multirow[c]{5}{*}{shared policy} & \multirow[c]{2}{*}{True} & 2 & 82.67 ± 3.06 & 47.90 ± 4.78 \\
 &  & 3 & 86.67 ± 3.51 & 48.80 ± 8.40 \\
\cline{2-5}
 & \multirow[c]{3}{*}{False} & 1 & 76.00 ± 12.77 & 32.13 ± 6.41 \\
 &  & 2 & 83.67 ± 9.61 & 45.33 ± 11.38 \\
 &  & 3 & 79.33 ± 11.85 & 38.13 ± 2.84 \\
\cline{1-5} \cline{2-5}
\bottomrule
\end{tabular}


% 10 eps

==> tables_OLD/obss_conv2_dungeon_eval_map_width_basic_stats_concise.tex <==
\begin{tabular}{lllll}
\toprule
 & \multicolumn{4}{r}{mean ep reward} \\
eval map width & 8 & 16 & 24 & 32 \\
obs size &  &  &  &  \\
\midrule
15 & 6.19 ± 0.34 & 38.48 ± 0.39 & 96.22 ± 2.07 & \textbf{140.16} ± \textbf{4.93} \\
20 & 7.06 ± 0.63 & 37.56 ± 1.93 & \textbf{97.18} ± \textbf{1.53} & 135.03 ± 2.04 \\
25 & \textbf{8.64} ± \textbf{1.74} & \textbf{39.44} ± \textbf{3.25} & 96.55 ± 0.78 & 136.51 ± 1.15 \\
31 & 7.51 ± 1.10 & 30.35 ± 3.35 & 91.37 ± 2.29 & 132.96 ± 5.16 \\
\bottomrule
\end{tabular}


==> tables_OLD/obswin.tex <==
\begin{tabular}{|c|c|c|c|}
\toprule
 &  & episode reward max & episode reward mean \\
model & task obs window &  &  \\
\midrule
\multirow[c]{5}{*}{SeqNCA} & (4, 4) & 159.67 ± 3.79 & \bfseries 98.74 ± 8.85 \\
 & (6, 6) & 159.33 ± 3.79 & 90.09 ± 7.22 \\
 & (8, 8) & 153.67 ± 18.23 & 98.09 ± 16.15 \\
 & (16, 16) & \bfseries 162.67 ± 6.43 & 95.53 ± 13.48 \\
 & (32, 32) & 159.67 ± 7.51 & 95.15 ± 15.63 \\
\cline{1-4}
\multirow[c]{5}{*}{Default} & (4, 4) & 65.33 ± 5.51 & 28.52 ± 2.21 \\
 & (6, 6) & 137.67 ± 12.58 & 86.25 ± 2.06 \\
 & (8, 8) & 143.33 ± 14.29 & 83.28 ± 1.95 \\
 & (16, 16) & 117.33 ± 7.77 & 67.84 ± 10.22 \\
 & (32, 32) & 106.33 ± 6.11 & 64.50 ± 8.02 \\
\cline{1-4}
\bottomrule
\end{tabular}


% 100 eps, but default 4x4 experiments haven't run for long enough!

==> tables_OLD/obswin_zelda.tex <==
\begin{tabular}{|c|c|c|c|c|}
\toprule
 &  &  & episode reward max & episode reward mean \\
task & model & task obs window &  &  \\
\midrule
\multirow[c]{10}{*}{zelda} & \multirow[c]{5}{*}{SeqNCA} & (4, 4) & 567.33 ± 47.88 & 371.33 ± 5.41 \\
 &  & (6, 6) & 625.67 ± 55.52 & 395.45 ± 13.81 \\
 &  & (8, 8) & 650.67 ± 58.16 & 408.00 ± 45.87 \\
 &  & (16, 16) & 625.00 ± 44.84 & 420.01 ± 20.25 \\
 &  & (32, 32) & \bfseries 685.67 ± 116.72 & \bfseries 433.42 ± 26.69 \\
\cline{2-5}
 & \multirow[c]{5}{*}{Default} & (4, 4) & 594.00 ± 42.51 & 383.09 ± 8.10 \\
 &  & (6, 6) & 490.00 ± 148.39 & 291.75 ± 137.42 \\
 &  & (8, 8) & 596.67 ± 18.90 & 386.28 ± 9.37 \\
 &  & (16, 16) & 618.33 ± 37.29 & 395.67 ± 4.36 \\
 &  & (32, 32) & 581.00 ± 29.05 & 404.47 ± 8.14 \\
\cline{1-5} \cline{2-5}
\bottomrule
\end{tabular}


==> tables_OLD/patch_width.tex <==
\begin{tabular}{|c|c|c|c|}
\toprule
 &  & episode reward max & episode reward mean \\
model & model patch width &  &  \\
\midrule
\multirow[c]{7}{*}{SeqNCA} & 3 & 159.67 ± 7.51 & 95.15 ± 15.63 \\
 & 5 & \bfseries 164.00 ± 6.24 & \bfseries 105.22 ± 18.33 \\
 & 7 & 149.33 ± 2.52 & 96.60 ± 5.26 \\
 & 9 & 146.33 ± 21.46 & 94.58 ± 12.87 \\
 & 11 & 131.33 ± 2.08 & 80.26 ± 2.88 \\
 & 16 & 98.33 ± 8.14 & 43.99 ± 0.71 \\
 & 32 & 98.00 ± 9.54 & 43.84 ± 4.64 \\
\cline{1-4}
\bottomrule
\end{tabular}


% 100 eps

==> tables_OLD/squeegee.tex <==
\begin{tabular}{|c|c|c|c|}
\toprule
 &  & episode reward max & episode reward mean \\
model & squeegee &  &  \\
\midrule
\multirow[c]{6}{*}{Default} & (16, 1) & \bfseries 132.00 ± 13.23 & \bfseries 95.94 ± 13.20 \\
 & (1, 16) & 126.00 ± 2.65 & 89.58 ± 3.56 \\
 & (8, 1) & 125.00 ± 13.45 & 88.91 ± 7.92 \\
 & (4, 1) & 110.00 ± 7.00 & 72.25 ± 6.89 \\
 & (2, 1) & 114.33 ± 8.50 & 69.02 ± 8.85 \\
 & (1, 1) & 98.33 ± 2.52 & 58.08 ± 1.49 \\
\cline{1-4}
\bottomrule
\end{tabular}

% 100 eps

==> tables_OLD/static_tiles.tex <==
\begin{tabular}{|c|c|c|c|c|}
\toprule
 &  &  & episode reward max & episode reward mean \\
model & static prob & freezies &  &  \\
\midrule
\multirow[c]{16}{*}{SeqNCA} & \multirow[c]{4}{*}{0.0} & 0 & \bfseries 142.00 ± 26.96 & \bfseries 105.83 ± 11.18 \\
 &  & 3 & 128.33 ± 15.89 & 72.60 ± 14.86 \\
 &  & 5 & 113.67 ± 6.66 & 70.70 ± 3.70 \\
 &  & 7 & 106.33 ± 10.50 & 70.50 ± 6.56 \\
\cline{2-5}
 & \multirow[c]{4}{*}{0.1} & 0 & 119.67 ± 13.65 & 72.20 ± 8.09 \\
 &  & 3 & 107.33 ± 15.31 & 72.80 ± 9.78 \\
 &  & 5 & 112.00 ± 8.89 & 63.67 ± 3.97 \\
 &  & 7 & 87.00 ± 18.25 & 55.07 ± 10.21 \\
\cline{2-5}
 & \multirow[c]{4}{*}{0.3} & 0 & 103.67 ± 16.01 & 59.60 ± 10.51 \\
 &  & 3 & 104.33 ± 14.47 & 63.40 ± 5.99 \\
 &  & 5 & 84.67 ± 0.58 & 56.37 ± 2.75 \\
 &  & 7 & 89.33 ± 16.01 & 48.57 ± 1.72 \\
\cline{2-5}
 & \multirow[c]{4}{*}{0.5} & 0 & 110.33 ± 12.10 & 56.60 ± 1.13 \\
 &  & 3 & 78.33 ± 17.50 & 49.30 ± 12.18 \\
 &  & 5 & 90.33 ± 7.09 & 46.43 ± 13.51 \\
 &  & 7 & 80.00 ± 8.89 & 38.87 ± 7.26 \\
\cline{1-5} \cline{2-5}
\bottomrule
\end{tabular}




==> tables_OLD/zelda.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\toprule
 &  & episode reward max & episode reward mean & episode reward min & path-length max & path-length mean & path-length min \\
model & task &  &  &  &  &  &  \\
\midrule
Default & zelda & 636.00 ± 37.24 & 412.93 ± 31.51 & 174.00 ± 38.74 & 33.00 ± 14.73 & 12.77 ± 12.46 & \bfseries 0.00 ± 0.00 \\
\cline{1-8}
SeqNCA & zelda & \bfseries 662.00 ± 101.34 & \bfseries 428.03 ± 27.88 & \bfseries 260.67 ± 27.59 & \bfseries 67.33 ± 40.50 & \bfseries 34.13 ± 30.53 & -0.67 ± 1.15 \\
\cline{1-8}
\bottomrule
\end{tabular}


% 100 eps
